PAC Best Arm Identification Under a Deadline

We study $(\epsilon, \delta)$-PAC best arm identification, where a decision-maker must identify an $\epsilon$-optimal arm with probability at least $1 - \delta$, while minimizing the number of arm pulls (samples). Most of the work on this topic is in the sequential setting, where there is no constraint on the time taken to identify such an arm; this allows the decision-maker to pull one arm at a time. In this work, the decision-maker is given a deadline of $T$ rounds, where, on each round, it can adaptively choose which arms to pull and how many times to pull them; this distinguishes the number of decisions made (i.e., time or number of rounds) from the number of samples acquired (cost). Such situations occur in clinical trials, where one may need to identify a promising treatment under a deadline while minimizing the number of test subjects, or in simulation-based studies run on the cloud, where we can elastically scale up or down the number of virtual machines to conduct as many experiments as we wish, but need to pay for the resource-time used. As the decision-maker can only make $T$ decisions, she may need to pull some arms excessively relative to a sequential algorithm in order to perform well on all possible problems. We formalize this added difficulty with two hardness results that indicate that unlike sequential settings, the ability to adapt to the problem difficulty is constrained by the finite deadline. We propose Elastic Batch Racing (EBR), a novel algorithm for this setting and bound its sample complexity, showing that EBR is optimal with respect to both hardness results. We present simulations evaluating EBR in this setting, where it outperforms baselines by several orders of magnitude.

==> note_to_reviewers.tex <==
\paragraph{A Note to the Reviewers:}
When writing up our proofs for the supplementary deadline, we discovered a mistake in one of our
intermediate technical lemmas; in particular,
we found that a certain result did not apply for general $n$.
Our updated manuscript makes the following changes to some results in Section~\ref{sec:lowerbound}.
% Unfortunately, this resulted in having to change one
% This changes some of the results, particularly in Section~\ref{sec:lowerbound},
% The main changes are:
\begin{itemize}
\item Theorem 3: the probabilistic lower bound now applies only for $n=2$ arms. The in-expectation
statement (which was previously part of Corollary 6) 
holds for arbitrary $n$ as it can be proved independently.
\item Theorem 5 and Corollary 6.2: This only holds only for $n=2$.
\item In addition, we have made some minor changes. This includes changes in the constants in
Theorem 4, 5, 6, a re-phrasing of the contributions to reflect the above changes, and other cosmetic
changes to refit into 8 pages.
\end{itemize}
We wish to emphasize that these changes do not significantly change the main take-aways of the
paper or the proof
intuitions for the lower bounds we had outlined in the original submission.
Moreover, they do not in any way affect the algorithm or the upper bounds.



